Gradient Descent in the Absence of Global Lipschitz Continuity of the Gradients

Gradient descent (GD) is a collection of continuous optimization methods that have achieved immeasurable success in practice. Owing to data science applications, GD with diminishing step sizes has become a prominent variant. While this variant of GD has been well-studied in the literature for objectives with globally Lipschitz continuous gradients or by requiring bounded iterates, objectives from data science problems do not satisfy such assumptions. Thus, in this work, we provide a novel global convergence analysis of GD with diminishing step sizes for differentiable nonconvex functions whose gradients are only locally Lipschitz continuous. Through our analysis, we generalize what is known about gradient descent with diminishing step sizes including interesting topological facts; and we elucidate the varied behaviors that can occur in the previously overlooked divergence regime. Thus, we provide the most general global convergence analysis of GD with diminishing step sizes under realistic conditions for data science problems.

==> figure/tikz-palis-de-melo-profile.tex <==
\begin{tikzpicture}[scale=2.0]

\node[anchor=north] at (0,1.25) {\tiny A Profile of the Palis-de Melo Function};

\draw[style=help lines] (-2,-1) grid (2,1);
\draw[blue,<->] (-2,0) to (2,0);
\node[blue,anchor=east] at (2,-0.1) {\tiny $\cmp{x}{1}$};
\draw[blue,<->] (0,-1) to (0,1);
\node[blue,anchor=west] at (0,0.9) {\tiny $F(x)$};

\draw[thick] plot [smooth] coordinates{
(-2.0, 0.6029403075542192)
(-1.99, 0.6040996409772953)
(-1.98, 0.6051915612841869)
(-1.97, 0.6062118901328637)
(-1.96, 0.6071562268146915)
(-1.95, 0.6080199362419088)
(-1.94, 0.6087981362893304)
(-1.93, 0.6094856844604137)
(-1.92, 0.6100771638475421)
(-1.91, 0.6105668683563571)
(-1.9, 0.6109487871642628)
(-1.89, 0.6112165883838941)
(-1.88, 0.6113636019034978)
(-1.87, 0.6113828013778945)
(-1.86, 0.6112667853461201)
(-1.85, 0.6110077574551188)
(-1.84, 0.6105975057731483)
(-1.83, 0.6100273811820798)
(-1.82, 0.6092882748447515)
(-1.81, 0.6083705947522697)
(-1.8, 0.6072642413669697)
(-1.79, 0.6059585823900606)
(-1.78, 0.6044424266992434)
(-1.77, 0.6027039975213694)
(-1.76, 0.6007309049291641)
(-1.75, 0.5985101177799288)
(-1.74, 0.5960279352488828)
(-1.73, 0.5932699581514985)
(-1.72, 0.5902210602990532)
(-1.71, 0.5868653601912032)
(-1.7, 0.5831861934204134)
(-1.69, 0.5791660862476322)
(-1.68, 0.574786730909115)
(-1.67, 0.5700289633336534)
(-1.66, 0.564872744091001)
(-1.65, 0.5592971435599842)
(-1.64, 0.5532803325032396)
(-1.63, 0.5467995794701784)
(-1.62, 0.5398312567269459)
(-1.61, 0.5323508567391938)
(-1.6, 0.5243330216189771)
(-1.59, 0.5157515884009065)
(-1.58, 0.5065796535462698)
(-1.57, 0.4967896607001897)
(-1.56, 0.4863535164609119)
(-1.55, 0.47524273977867193)
(-1.54, 0.46342865160291863)
(-1.53, 0.4508826125612786)
(-1.52, 0.4375763178032879)
(-1.51, 0.42348215969908937)
(-1.5, 0.40857367087003865)
(-1.49, 0.3928260620642397)
(-1.48, 0.37621687168995177)
(-1.47, 0.3587267463882847)
(-1.46, 0.340340374851964)
(-1.45, 0.32104760014117184)
(-1.44, 0.30084473893193886)
(-1.43, 0.2797361393174265)
(-1.42, 0.2577360117371835)
(-1.41, 0.23487056997134625)
(-1.4, 0.21118052035223847)
(-1.39, 0.18672393658923267)
(-1.38, 0.16157955366376892)
(-1.37, 0.13585050538187418)
(-1.36, 0.10966851387887269)
(-1.35, 0.08319851214592118)
(-1.34, 0.05664363761367131)
(-1.33, 0.030250469306321782)
(-1.32, 0.004314284084269766)
(-1.31, -0.02081603278926467)
(-1.3, -0.04473398614307192)
(-1.29, -0.06697321707873088)
(-1.28, -0.08700820782580074)
(-1.27, -0.10425964536525788)
(-1.26, -0.11810676123303933)
(-1.25, -0.12790969883957673)
(-1.24, -0.13304574696055196)
(-1.23, -0.1329639525204073)
(-1.22, -0.12726283045257622)
(-1.21, -0.11579493608361743)
(-1.2, -0.09879873847753255)
(-1.19, -0.07705054971598181)
(-1.18, -0.05201435319611254)
(-1.17, -0.0259418870034577)
(-1.16, -0.0018374985330704573)
(-1.15, 0.016842153517095733)
(-1.14, 0.02690761512438477)
(-1.13, 0.02666139529939691)
(-1.12, 0.017415470031541033)
(-1.11, 0.0044088460911617935)
(-1.1, -0.004651004840475783)
(-1.09, -0.004878046792010928)
(-1.08, -0.00016282239634929648)
(-1.07, 0.0009953807574970318)
(-1.06, -0.00025077329998062094)
(-1.05, 5.2896312553892364e-5)
(-1.04, -6.302217546888124e-7)
(-1.03, 6.951846536832215e-8)
(-1.02, -4.6672256222854166e-12)
(-1.01, -1.2524880399776846e-22)
(-1.0, 0)
(-0.99, 1.5002260015546792e-22)
(-0.98, 1.0788663030635898e-11)
(-0.97, 4.4826167446000153e-8)
(-0.96, 2.8875503621930564e-6)
(-0.95, 3.5131575098565605e-5)
(-0.94, 0.00018575809558309835)
(-0.93, 0.0006100775361876936)
(-0.92, 0.0014878596523651834)
(-0.91, 0.002975522395517596)
(-0.9, 0.005178924370597747)
(-0.89, 0.008147820506529896)
(-0.88, 0.011883265685449677)
(-0.87, 0.01634989955147807)
(-0.86, 0.02148831938865155)
(-0.85, 0.027225435782070338)
(-0.84, 0.03348227346715186)
(-0.83, 0.04017941358888236)
(-0.82, 0.04724053075146394)
(-0.81, 0.05459450505625923)
(-0.8, 0.062176524022116264)
(-0.79, 0.0699284998340553)
(-0.78, 0.07779904296210309)
(-0.77, 0.08574316374671881)
(-0.76, 0.09372182033358106)
(-0.75, 0.10170139230422684)
(-0.74, 0.10965313156124244)
(-0.73, 0.11755262269950272)
(-0.72, 0.1253792719208833)
(-0.71, 0.13311583474782598)
(-0.7, 0.1407479870412307)
(-0.69, 0.14826394017771144)
(-0.68, 0.15565409901507965)
(-0.67, 0.16291076000099322)
(-0.66, 0.17002784613167035)
(-0.65, 0.1770006752220519)
(-0.64, 0.18382575795440456)
(-0.63, 0.19050062232762832)
(-0.62, 0.19702366136735677)
(-0.61, 0.20339400123366172)
(-0.6, 0.2096113871510978)
(-0.59, 0.21567608486793102)
(-0.58, 0.22158879561781497)
(-0.57, 0.22735058280271436)
(-0.56, 0.23296280883833387)
(-0.55, 0.23842708080241162)
(-0.54, 0.2437452037028098)
(-0.53, 0.24891914033788473)
(-0.52, 0.25395097685792606)
(-0.51, 0.2588428932554536)
(-0.5, 0.26359713811572677)
(-0.49, 0.2682160070487578)
(-0.48, 0.27270182430209833)
(-0.47, 0.27705692712118063)
(-0.46, 0.28128365248241405)
(-0.45, 0.28538432587473733)
(-0.44, 0.28936125184899175)
(-0.43, 0.29321670609220163)
(-0.42, 0.2969529288164625)
(-0.41, 0.30057211928031297)
(-0.4, 0.30407643128483336)
(-0.39, 0.3074679695077815)
(-0.38, 0.31074878655729843)
(-0.37, 0.3139208806424898)
(-0.36, 0.3169861937718391)
(-0.35, 0.3199466104022343)
(-0.34, 0.32280395647163374)
(-0.33, 0.3255599987572783)
(-0.32, 0.32821644450905824)
(-0.31, 0.33077494131432317)
(-0.3, 0.33323707715622386)
(-0.29, 0.3356043806327085)
(-0.28, 0.3378783213076668)
(-0.27, 0.3400603101695161)
(-0.26, 0.34215170017582136)
(-0.25, 0.34415378686541237)
(-0.24, 0.3460678090219527)
(-0.23, 0.34789494937508164)
(-0.22, 0.34963633532713745)
(-0.21, 0.351293039695104)
(-0.2, 0.3528660814588489)
(-0.19, 0.3543564265079545)
(-0.18, 0.3557649883805202)
(-0.17, 0.35709262898824357)
(-0.16, 0.35834015932289764)
(-0.15, 0.35950834014002236)
(-0.14, 0.36059788261625575)
(-0.13, 0.3616094489772548)
(-0.12, 0.36254365309361164)
(-0.11, 0.3634010610425608)
(-0.1, 0.3641821916336149)
(-0.09, 0.36488751689655263)
(-0.08, 0.36551746253043926)
(-0.07, 0.36607240831257165)
(-0.06, 0.36655268846642575)
(-0.05, 0.36695859198784514)
(-0.04, 0.36729036292884537)
(-0.03, 0.3675482006385271)
(-0.02, 0.3677322599606948)
(-0.01, 0.3678426513878667)
(0.0, 0.36787944117144233)
(0.01, 0.3678426513878667)
(0.02, 0.3677322599606948)
(0.03, 0.3675482006385271)
(0.04, 0.36729036292884537)
(0.05, 0.36695859198784514)
(0.06, 0.36655268846642575)
(0.07, 0.36607240831257165)
(0.08, 0.36551746253043926)
(0.09, 0.36488751689655263)
(0.1, 0.3641821916336149)
(0.11, 0.3634010610425608)
(0.12, 0.36254365309361164)
(0.13, 0.3616094489772548)
(0.14, 0.36059788261625575)
(0.15, 0.35950834014002236)
(0.16, 0.35834015932289764)
(0.17, 0.35709262898824357)
(0.18, 0.3557649883805202)
(0.19, 0.3543564265079545)
(0.2, 0.3528660814588489)
(0.21, 0.351293039695104)
(0.22, 0.34963633532713745)
(0.23, 0.34789494937508164)
(0.24, 0.3460678090219527)
(0.25, 0.34415378686541237)
(0.26, 0.34215170017582136)
(0.27, 0.3400603101695161)
(0.28, 0.3378783213076668)
(0.29, 0.3356043806327085)
(0.3, 0.33323707715622386)
(0.31, 0.33077494131432317)
(0.32, 0.32821644450905824)
(0.33, 0.3255599987572783)
(0.34, 0.32280395647163374)
(0.35, 0.3199466104022343)
(0.36, 0.3169861937718391)
(0.37, 0.3139208806424898)
(0.38, 0.31074878655729843)
(0.39, 0.3074679695077815)
(0.4, 0.30407643128483336)
(0.41, 0.30057211928031297)
(0.42, 0.2969529288164625)
(0.43, 0.29321670609220163)
(0.44, 0.28936125184899175)
(0.45, 0.28538432587473733)
(0.46, 0.28128365248241405)
(0.47, 0.27705692712118063)
(0.48, 0.27270182430209833)
(0.49, 0.2682160070487578)
(0.5, 0.26359713811572677)
(0.51, 0.2588428932554536)
(0.52, 0.25395097685792606)
(0.53, 0.24891914033788473)
(0.54, 0.2437452037028098)
(0.55, 0.23842708080241162)
(0.56, 0.23296280883833387)
(0.57, 0.22735058280271436)
(0.58, 0.22158879561781497)
(0.59, 0.21567608486793102)
(0.6, 0.2096113871510978)
(0.61, 0.20339400123366172)
(0.62, 0.19702366136735677)
(0.63, 0.19050062232762832)
(0.64, 0.18382575795440456)
(0.65, 0.1770006752220519)
(0.66, 0.17002784613167035)
(0.67, 0.16291076000099322)
(0.68, 0.15565409901507965)
(0.69, 0.14826394017771144)
(0.7, 0.1407479870412307)
(0.71, 0.13311583474782598)
(0.72, 0.1253792719208833)
(0.73, 0.11755262269950272)
(0.74, 0.10965313156124244)
(0.75, 0.10170139230422684)
(0.76, 0.09372182033358106)
(0.77, 0.08574316374671881)
(0.78, 0.07779904296210309)
(0.79, 0.0699284998340553)
(0.8, 0.062176524022116264)
(0.81, 0.05459450505625923)
(0.82, 0.04724053075146394)
(0.83, 0.04017941358888236)
(0.84, 0.03348227346715186)
(0.85, 0.027225435782070338)
(0.86, 0.02148831938865155)
(0.87, 0.01634989955147807)
(0.88, 0.011883265685449677)
(0.89, 0.008147820506529896)
(0.9, 0.005178924370597747)
(0.91, 0.002975522395517596)
(0.92, 0.0014878596523651834)
(0.93, 0.0006100775361876936)
(0.94, 0.00018575809558309835)
(0.95, 3.5131575098565605e-5)
(0.96, 2.8875503621930564e-6)
(0.97, 4.4826167446000153e-8)
(0.98, 1.0788663030635898e-11)
(0.99, 1.5002260015546792e-22)
(1.0, 0)
(1.01, 1.2524880399776846e-22)
(1.02, 4.6672256222854166e-12)
(1.03, -6.951846536832215e-8)
(1.04, 6.302217546888124e-7)
(1.05, -5.2896312553892364e-5)
(1.06, 0.00025077329998062094)
(1.07, -0.0009953807574970318)
(1.08, 0.00016282239634929648)
(1.09, 0.004878046792010928)
(1.1, 0.004651004840475783)
(1.11, -0.0044088460911617935)
(1.12, -0.017415470031541033)
(1.13, -0.02666139529939691)
(1.14, -0.02690761512438477)
(1.15, -0.016842153517095733)
(1.16, 0.0018374985330704573)
(1.17, 0.0259418870034577)
(1.18, 0.05201435319611254)
(1.19, 0.07705054971598181)
(1.2, 0.09879873847753255)
(1.21, 0.11579493608361743)
(1.22, 0.12726283045257622)
(1.23, 0.1329639525204073)
(1.24, 0.13304574696055196)
(1.25, 0.12790969883957673)
(1.26, 0.11810676123303933)
(1.27, 0.10425964536525788)
(1.28, 0.08700820782580074)
(1.29, 0.06697321707873088)
(1.3, 0.04473398614307192)
(1.31, 0.02081603278926467)
(1.32, -0.004314284084269766)
(1.33, -0.030250469306321782)
(1.34, -0.05664363761367131)
(1.35, -0.08319851214592118)
(1.36, -0.10966851387887269)
(1.37, -0.13585050538187418)
(1.38, -0.16157955366376892)
(1.39, -0.18672393658923267)
(1.4, -0.21118052035223847)
(1.41, -0.23487056997134625)
(1.42, -0.2577360117371835)
(1.43, -0.2797361393174265)
(1.44, -0.30084473893193886)
(1.45, -0.32104760014117184)
(1.46, -0.340340374851964)
(1.47, -0.3587267463882847)
(1.48, -0.37621687168995177)
(1.49, -0.3928260620642397)
(1.5, -0.40857367087003865)
(1.51, -0.42348215969908937)
(1.52, -0.4375763178032879)
(1.53, -0.4508826125612786)
(1.54, -0.46342865160291863)
(1.55, -0.47524273977867193)
(1.56, -0.4863535164609119)
(1.57, -0.4967896607001897)
(1.58, -0.5065796535462698)
(1.59, -0.5157515884009065)
(1.6, -0.5243330216189771)
(1.61, -0.5323508567391938)
(1.62, -0.5398312567269459)
(1.63, -0.5467995794701784)
(1.64, -0.5532803325032396)
(1.65, -0.5592971435599842)
(1.66, -0.564872744091001)
(1.67, -0.5700289633336534)
(1.68, -0.574786730909115)
(1.69, -0.5791660862476322)
(1.7, -0.5831861934204134)
(1.71, -0.5868653601912032)
(1.72, -0.5902210602990532)
(1.73, -0.5932699581514985)
(1.74, -0.5960279352488828)
(1.75, -0.5985101177799288)
(1.76, -0.6007309049291641)
(1.77, -0.6027039975213694)
(1.78, -0.6044424266992434)
(1.79, -0.6059585823900606)
(1.8, -0.6072642413669697)
(1.81, -0.6083705947522697)
(1.82, -0.6092882748447515)
(1.83, -0.6100273811820798)
(1.84, -0.6105975057731483)
(1.85, -0.6110077574551188)
(1.86, -0.6112667853461201)
(1.87, -0.6113828013778945)
(1.88, -0.6113636019034978)
(1.89, -0.6112165883838941)
(1.9, -0.6109487871642628)
(1.91, -0.6105668683563571)
(1.92, -0.6100771638475421)
(1.93, -0.6094856844604137)
(1.94, -0.6087981362893304)
(1.95, -0.6080199362419088)
(1.96, -0.6071562268146915)
(1.97, -0.6062118901328637)
(1.98, -0.6051915612841869)
(1.99, -0.6040996409772953)
(2.0, -0.6029403075542192)
};

\node[purple] (A) at (1.159,0) {\tiny\textbullet};
\node[purple,anchor=north] (Alab) at (1.159,-0.3) {\tiny $1 + 1/(2\pi)$};
\draw [purple,->] (Alab) to (A);

\node[purple] (B) at (1.318,0) {\tiny\textbullet};
\node[purple,anchor=west] (Blab) at (1.318,0.3) {\tiny $1+1/\pi$};
\draw[purple,->] (Blab) to (B);

\end{tikzpicture}

==> figure/tikz-palis-de-melo.tex <==
\begin{tikzpicture}

\node[anchor=north] at (0,2.5) {\tiny Zero Set of the Palis-de Melo Function};

\draw[style=help lines] (-4,-2) grid (4,2);
\draw[blue,<->] (-4,0) to (4,0);
\node[blue,anchor=east] at (4,-0.2) {\tiny $\cmp{x}{1}$};
\draw[blue,<->] (0,-2) to (0,2);
\node[blue,anchor=west] at (0,1.85) {\tiny $\cmp{x}{2}$};

\node at (-3.5,1.5) {\tiny +};
\node at (-3.5,0.5) {\tiny +};
\node at (-3.5,-0.5) {\tiny +};
\node at (-2.5,1.5) {\tiny +};
\node at (-2.5,0.5) {\tiny +};
\node at (-2.5,-0.5) {\tiny +};
\node at (-2.5,-1.25) {\tiny +};
\node at (-1.5,1.5) {\tiny +};
\node at (-1.6,0.5) {\tiny +};
\node at (-1.5,-0.5) {\tiny +};
\node at (-1.5,-1.35) {\tiny +};
\node at (-0.5,-1.45) {\tiny +};
\node at (-0.5, 1.75) {\tiny +};
\node at (1.5, 1.85) {\tiny +};
\node at (2.5, 1.75) {\tiny +};
\node at (3.5, 1.6) {\tiny +};

\node[red] at (-3.5,-1.6) {-};
\node[red] at (-2.5,-1.75) {-};
\node[red] at (-1.5,-1.85) {-};
\node[red] at (0.5,-1.75) {-};
\node[red] at (0.5,1.45) {-};
\node[red] at (1.5,1.35) {-};
\node[red] at (1.5,0.5) {-};
\node[red] at (1.6,-0.5) {-};
\node[red] at (1.5,-1.5) {-};
\node[red] at (2.5,1.25) {-};
\node[red] at (2.5,0.5) {-};
\node[red] at (2.5,-0.5) {-};
\node[red] at (2.5,-1.5) {-};
\node[red] at (3.5, 0.5) {-};
\node[red] at (3.5,-0.5) {-};
\node[red] at (3.5,-1.5) {-};

\node at (-0.4,0.4) {\tiny + };
\node at (-0.4,-0.4) {\tiny +};
\node at (0.4,0.4) {\tiny +};
\node at (0.4,-0.4) {\tiny +};

\path [draw=green] (0,0) circle (1cm);

\draw[name path=upper] plot [smooth] coordinates{
(3.9783634308577818, 1.2926486374584134)
(2.0966075313761574, 1.5232745360811122)
(1.2114447748182324, 1.6674106857090871)
(0.5549249051458139, 1.7078832449358106)
(1.0021405828256142e-16, 1.6366197723675815)
(-0.47295560155552496, 1.4556076687222583)
(-0.8550679048035127, 1.1769000049467218)
(-1.1309146286252498, 0.8216575732396331)
(-1.2874239512465566, 0.41830939916199933)
(-1.3183098861837907, 1.614463982399291e-16)
(-1.226266235800847, -0.3984380528370805)
(-1.0236154172084824, -0.7437001329239128)
(-0.7317066805676485, -1.0071078462212875)
(-0.379276397452338, -1.1672927244781983)
(-2.226787381972967e-16, -1.2122065907891937)
(0.37049397206766377, -1.1402631984553178)
(0.6978428150911363, -0.9604982340221487)
(0.9520826095973038, -0.6917285060467666)
(1.110388459166871, -0.36078708085302486)
(1.1591549430918953, -2.839110781546644e-16)
(1.0952139884171834, 0.3558565964265407)
(0.9260706795568757, 0.6728297326368946)
(0.6691321465349638, 0.9209813888967915)
(0.35000164617009216, 1.0771943044019296)
(3.4514341811203206e-16, 1.1273239544735163)
(-0.3468489806473881, 1.0674913976244855)
(-0.657080754795335, 0.9043940711898519)
(-0.9009877470178907, 0.6546059154202333)
(-1.0554464099007612, 0.34293532689506734)
(-1.1061032953945968, 4.063757580693997e-16)
(-1.0487115780552383, -0.34074704737763944)
(-0.8894914029375233, -0.6462533325292626)
(-0.644481572522088, -0.8870527844962327)
(-0.33794733681857925, -1.0400949549587601)
(-4.676080980267674e-16, -1.0909456817667973)
(0.3363400955717099, -1.0351483750330046)
(0.6383522406053721, -0.8786164828614995)
(0.8767849173750109, -0.6370215303866125)
(1.028679770514708, -0.3342383185565752)
(1.0795774715459476, -5.28840437984135e-16)
(1.0248932703088764, 0.33300801005990954)
(0.8703308294702434, 0.6323323610443126)
(0.631296381771015, 0.8689049263284918)
(0.33137225899048134, 1.0198589461715768)
(5.900727779415027e-16, 1.0707355302630646)
(-0.33040029096371787, 1.0168675361769501)
(-0.6275933069217765, 0.8638080810558504)
(-0.8626666000833308, 0.6267639724503336)
(-1.0128382900617376, 0.3290911095399167)
(-1.0636619772367581, 6.513051178988704e-16)
(-1.0104154754042256, -0.3283038893373659)
(-0.8585397073365327, -0.6237656093612663)
(-0.6230867346995906, -0.8576053165259373)
(-0.32723239517279007, -1.0071177554537205)
(-2.591700105142178e-15, -1.0578745247606893)
(0.32658184514429434, -1.005115568340915)
(0.6206094376885667, -0.8541956097083225)
(0.8534166680646439, -0.6200435034575992)
(1.002366802982655, -0.3256887171390765)
(1.0530516476972984, -7.737697978136056e-16)
(1.0006844985010979, 0.32514210327795606)
(0.8505521729878902, 0.6179623259630738)
(0.6174833247937018, 0.8498928844384762)
(0.32438623879812734, 0.9983581868351943)
(-1.0283442313787065e-15, 1.048970751720583)
(-0.32392050411863554, 0.9969248028794362)
(-0.615710305539893, 0.8474525327928957)
(-0.8468873042867472, 0.6152996429921397)
(-0.9949305295496846, 0.32327252543412716)
(-1.0454728408833986, 8.962344777283409e-16)
(-0.9936946418523745, -0.32287096117893727)
(-0.844783398180537, -0.6137710657310458)
(-0.613415095683942, -0.8442934474434742)
(-0.32230931387607625, -0.9919660691946484)
};

\draw[name path=lower,orange] plot [smooth] coordinates{
(-3.9783634308577818, -1.2926486374584139)
(-2.096607531376157, -1.5232745360811126)
(-1.2114447748182322, -1.6674106857090871)
(-0.5549249051458138, -1.7078832449358108)
(1.0021405828256142e-16, -1.6366197723675815)
(0.47295560155552513, -1.455607668722258)
(0.8550679048035129, -1.1769000049467218)
(1.1309146286252498, -0.821657573239633)
(1.2874239512465566, -0.41830939916199916)
(1.3183098861837907, 0.0)
(1.226266235800847, 0.3984380528370806)
(1.0236154172084824, 0.7437001329239129)
(0.7317066805676484, 1.0071078462212875)
(0.3792763974523379, 1.1672927244781983)
(7.422624606576558e-17, 1.2122065907891937)
(-0.37049397206766393, 1.1402631984553178)
(-0.6978428150911364, 0.9604982340221486)
(-0.9520826095973038, 0.6917285060467665)
(-1.110388459166871, 0.3607870808530247)
(-1.1591549430918953, 1.419555390773322e-16)
(-1.0952139884171834, -0.3558565964265409)
(-0.9260706795568756, -0.6728297326368947)
(-0.6691321465349636, -0.9209813888967916)
(-0.350001646170092, -1.0771943044019296)
(-2.0708605086721922e-16, -1.1273239544735163)
(0.3468489806473882, -1.0674913976244855)
(0.657080754795335, -0.9043940711898519)
(0.9009877470178909, -0.6546059154202333)
(1.0554464099007612, -0.3429353268950671)
(1.1061032953945968, -2.7091717204626647e-16)
(1.0487115780552383, 0.3407470473776396)
(0.8894914029375232, 0.6462533325292628)
(0.6444815725220879, 0.8870527844962327)
(0.33794733681857914, 1.0400949549587604)
(3.3400578430483383e-16, 1.0909456817667973)
(-0.33634009557171, 1.0351483750330044)
(-0.6383522406053723, 0.8786164828614994)
(-0.876784917375011, 0.6370215303866124)
(-1.028679770514708, 0.3342383185565751)
(-1.0795774715459476, 3.966303284881012e-16)
(-1.0248932703088764, -0.33300801005990965)
(-0.8703308294702433, -0.6323323610443127)
(-0.6312963817710149, -0.8689049263284919)
(-0.3313722589904812, -1.0198589461715768)
(-4.58945493954502e-16, -1.0707355302630646)
(0.33040029096371804, -1.0168675361769501)
(0.6275933069217766, -0.8638080810558503)
(0.8626666000833308, -0.6267639724503334)
(1.0128382900617376, -0.3290911095399166)
(1.0636619772367581, -5.210440943190963e-16)
(1.0104154754042256, 0.328303889337366)
(0.8585397073365327, 0.6237656093612665)
(0.6230867346995905, 0.8576053165259373)
(0.32723239517278996, 1.0071177554537205)
(2.4621478400774077e-15, 1.0578745247606893)
(-0.32658184514429445, 1.005115568340915)
(-0.6206094376885668, 0.8541956097083224)
(-0.853416668064644, 0.6200435034575991)
(-1.0023668029826551, 0.3256887171390764)
(-1.0530516476972984, 6.448081648446714e-16)
(-1.0006844985010979, -0.3251421032779562)
(-0.8505521729878901, -0.6179623259630739)
(-0.6174833247937018, -0.8498928844384764)
(-0.3243862387981272, -0.9983581868351945)
(1.156806098728087e-15, -1.048970751720583)
(0.32392050411863565, -0.9969248028794361)
};

\node[purple] (A) at (1.159,0) {\tiny\textbullet};
\node[purple] (B) at (1.318,0) {\tiny\textbullet};

\end{tikzpicture}

==> section/continuous-approximation.tex <==
The continuous approximation of gradient descent uses continuous gradient descent to approximate the behavior of (stochastic) gradient descent methods with diminishing step sizes. Under certain conditions \cite{ljung1977,benaim1999,benveniste2012,mertikopoulos2020}, the continuous approximation of gradient descent can lead to appropriate conclusions. However, the continuous approximation is not always appropriate. Indeed, as we show in this section, there exists a function satisfying \cref{assumption-lower-bound,assumption-gradient} for which continuous gradient descent will have an asymptotic solution that cannot occur for gradient descent with diminishing step sizes.

To establish this result, we begin by reviewing continuous gradient descent. We then discuss a particular limiting behavior for continuous gradient descent, limit cycles, and a modification of a classical objective function satisfying \cref{assumption-lower-bound,assumption-gradient} for which continuous gradient descent has a limit cycle. We then prove that gradient descent with diminishing step sizes satisfying \cref{property-summable} cannot have this limit cycle. Note, while we can prove this statement as a simple consequence of \cref{result-zoutendjik-summable}, we will supply geometric intuition.


\subsection{Continuous Gradient Descent}
Let $x \in \mathbb{R}^p$ be arbitrary. Consider the initial value problem,
\begin{equation} \label{eqn-ivp}
\begin{cases}
\frac{dy}{dt} &= - \dot F(y(t)), ~ t \geq 0 \\
y(0) &= x.
\end{cases}
\end{equation}
To explicitly show the dependence on the initial value, $x$, we will write $\Phi_h(x)$ to be the solution (if it exists) to \cref{eqn-ivp} at time $h \geq 0$ that is initialized at $x \in \mathbb{R}^p$. If $F$ satisfies \cref{assumption-gradient}, we can apply the Picard-Lindel\"{o}f theorem to conclude that $\Phi_h(x)$ exists and is unique for any finite, non-negative choice of $h$. Therefore, we define continuous gradient descent initialized at $x \in \mathbb{R}^p$ to be $\lbrace \Phi_h(x) : h \geq 0 \rbrace$.

\subsection{Limit Cycles of Continuous Gradient Descent}
There are many possible choices for the asymptotics of continuous gradient descent; two particularly interesting cases are cycles and limit cycles. Recall, a cycle cannot be a solution for continuous gradient descent. To see why, suppose such a cycle exists and $x$ is a point on this cycle. Then there would exist a $t > 0$ such that $F(\Phi_t(x)) = F(x)$, but
\begin{equation*}
0 = F(\Phi_t(x)) - F(x) = \int_0^t \dot F(\Phi_s(x))^\intercal \left( \frac{d}{dr} \Phi_r(x) \vert_{r=s} \right) ds = \int_0^t - \norm{ \dot F(\Phi_s(x))}_2^2 ds < 0.
\end{equation*}
Hence, a cycle cannot be a solution for continuous gradient descent. 

However, it is possible for continuous gradient descent to have a limit cycle. To see how, consider a small modification of the Palis-de Melo function \cite[\S 1, Example 3]{palis2012}, $F: \mathbb{R}^2 \to \mathbb{R}$, specified by
\begin{equation} \label{eqn-pdm}
F(x) = \begin{cases}
\exp\left(\frac{1}{\norm{x}_2^2 - 1}  \right) & \norm{x}_2 < 1 \\
0 & \norm{x}_2 = 1 \\
-\exp\left(\frac{-1}{\norm{x}_2^2 - 1} \right) \left[ \sin\left( \frac{1}{\norm{x}_2-1}  \right) \frac{\cmp{x}{1}}{\norm{x}_2} -  \cos\left( \frac{1}{\norm{x}_2-1}  \right) \frac{\cmp{x}{2}}{\norm{x}_2} \right] & \norm{x}_2 > 1,
\end{cases}
\end{equation}
where $\cmp{x}{j}$ is the $j^\mathrm{th}$ component of $x$. The zero set of the Palis-de Melo function is plotted in \cref{figure-palis-de-melo-zero}, and a profile of the function when $\cmp{x}{2} = 0$ is plotted in \cref{figure-palis-de-melo-profile}. Importantly, the Palis-de Melo function satisfies \cref{assumption-lower-bound,assumption-gradient}.

\begin{proposition} \label{result-pdm-assumptions}
The Palis-de Melo function, \cref{eqn-pdm}, is bounded from below, is differentiable at every point in $\mathbb{R}^2$, and its gradient is locally Lipschitz continuous at every point in $\mathbb{R}^2$. 
\end{proposition}
\begin{proof}
To verify that the Palis-de Melo function is bounded from below, we look at the three components separately. When $\inlinenorm{x}_2 < 1$, $F(x) \geq 0$. When $\inlinenorm{x}_2 = 1$, $F(x) = 0$. When $\inlinenorm{x}_2 > 1$, define
\begin{equation}
\theta = \begin{cases}
\arcsin\left( \frac{\cmp{x}{2}}{\norm{x}_2} \right) & \cmp{x}{1} \geq 0 \\
\pi - \arcsin\left( \frac{\cmp{x}{2}}{\norm{x}_2} \right) & \cmp{x}{1} < 0
\end{cases}
\end{equation}
Then, when $\inlinenorm{x}_2 > 1$,
\begin{equation}
F(x) = - \exp\left(\frac{-1}{\norm{x}_2^2 - 1} \right) \sin\left( \frac{1}{\norm{x}_2 -1} - \theta \right) \geq - \exp\left(\frac{-1}{\norm{x}_2^2 - 1} \right) \geq -1.
\end{equation}
Thus, $F$ is bounded from below.

We now show that $F$ is continuously differentiable. When $\inlinenorm{x}_2 < 1$, we can differentiate to conclude
\begin{equation}
\dot F(x) = \exp\left( \frac{1}{\norm{x}_2^2 - 1} \right) \frac{-2}{\left( \norm{x}_2^2 - 1  \right)^2} x.
\end{equation}
Next, let $x \in \mathbb{R}^2$ such that $\inlinenorm{x}_2 = 1$. Then,
\begin{equation}
\dot F(x) = \lim_{x_n \to x} \frac{|F(x_n)|}{\norm{x_n - x}_2} \leq \lim_{x_n \to x } \frac{\min\left\lbrace \exp\left( \frac{1}{\norm{x_n}_2^2 -1 }  \right),\exp\left( \frac{-1}{\norm{x_n}_2^2 -1 }  \right) \right\rbrace}{\norm{x_n - x}_2} = 0.
\end{equation}
When $\inlinenorm{x}_2 > 1$, we can differentiate to conclude
\begin{equation*}
\begin{aligned}
\dot F(x) & = 
\exp\left( \frac{-1}{\norm{x}_2^2 - 1} \right) \frac{2}{\left( \norm{x}_2^2 - 1  \right)^2}  \left[ \sin\left( \frac{1}{\norm{x}_2-1}  \right) \frac{\cmp{x}{1}}{\norm{x}_2} -  \cos\left( \frac{1}{\norm{x}_2-1}  \right) \frac{\cmp{x}{2}}{\norm{x}_2} \right]x \\
&\quad + 
\exp\left( \frac{-1}{\norm{x}_2^2 - 1} \right)\left[ 
\frac{-\cmp{x}{1}}{(\norm{x}_2 - 1)^2 \norm{x}_2^2}  \cos\left( \frac{1}{\norm{x}_2-1}  \right) x 
- \sin\left( \frac{1}{\norm{x}_2-1}  \right)\frac{\cmp{x}{1}}{\norm{x}_2^3}x \right. \\
&\quad + \sin\left( \frac{1}{\norm{x}_2-1}  \right) \frac{1}{\norm{x}_2}\begin{bmatrix} 1 \\ 0 \end{bmatrix} 
-\frac{\cmp{x}{2}}{(\norm{x}_2 - 1)^2 \norm{x}_2^2}  \sin\left( \frac{1}{\norm{x}_2-1}  \right) x  \\
&\quad \left. + \cos\left( \frac{1}{\norm{x}_2-1}  \right)\frac{\cmp{x}{2}}{\norm{x}_2^3}x
-\cos\left( \frac{1}{\norm{x}_2-1}  \right) \frac{1}{\norm{x}_2}\begin{bmatrix} 0 \\ 1 \end{bmatrix}\right].
\end{aligned}
\end{equation*}
Finally, notice that when when $\norm{x}_2$ is near $1$, $\dot F(x)$ is dominated by the exponential term which goes to zero. Hence, $\dot F$ is continuously differentiable.

We can do the identical, yet more tedious calculation to conclude that the second derivative of $F(x)$ exists for all $x \in \mathbb{R}^2$ and is continuous. We can then apply \cref{result-hessian-implies-lipschitz} to conclude that $\dot F(x)$ is locally Lipschitz continuous.
\end{proof}

By \cref{result-pdm-assumptions}, continuous gradient descent is well-defined on the Palis-de Melo function. There is an appropriate initialization of continuous gradient descent that results in a path whose limit cycle is the circle of radius one, which we show next.

\begin{proposition} \label{result-pdm-limit-cycle}
Let $\mathcal{S} = \lbrace z \in \mathbb{R}^2 : \inlinenorm{z}_2 = 1 \rbrace$. Let $\lbrace \Phi_t(x): t \geq 0 \rbrace$ denote continuous gradient descent on \cref{eqn-pdm} when initialized at $x \in \mathbb{R}^2$. Let
\begin{equation}
\mathcal{U} = \left\lbrace \begin{bmatrix} r\cos(\theta) \\ r \sin(\theta) \end{bmatrix}: ~r\geq 0, ~\theta \geq 0, 1+ \frac{1}{2\pi+\theta} < r < 1 + \frac{1}{\pi + \theta}  \right\rbrace \subset \mathbb{R}^2.
\end{equation}
There exists an $x \in \mathbb{R}^2$ for which $\cmp{x}{1} \in (1+\frac{1}{2\pi}, 1 + \frac{1}{\pi})$ and $\cmp{x}{2} = 0$ such that $\Phi_h(x) \in \mathcal{U}$ for all $h \geq 0$. Moreover, for all $ z \in \mathcal{S}$,  $\exists \lbrace t_i : i \in \mathbb{N} \rbrace \subset \mathbb{R}_{\geq 0}$ such that $\lim_{i \to \infty} \Phi_{t_i}(x) = z$.
\end{proposition}
\begin{proof}
The proof is a small modification of that given in \cite[\S 1, Example 3]{palis2012}.
\end{proof}

The basic idea of the proof is best understood geometrically. Consider the initialization of continuous gradient descent between the purple points in \cref{figure-palis-de-melo-zero} (equivalently, \cref{figure-palis-de-melo-profile}). From \cref{figure-palis-de-melo-profile}, the initialization is in a region where the objective function is positive. Hence, as continuous gradient descent attempts to reduce the objective function value, continuous gradient descent initialized in this region should go towards the black spiral or orange spiral in \cref{figure-palis-de-melo-zero}, or towards another point between the purple points in \cref{figure-palis-de-melo-zero}. Hence, by the Picard-Lindel\"{o}f theorem (which can be applied by \cref{result-pdm-assumptions}), there is a point between the set of initializations going towards the black spiral and the other two alternatives. Thus, if continuous gradient descent is initialized at one of these points, it must remain between the black and orange spirals (i.e., stay within $\mathcal{U}$) and must have a limit cycle of $\mathcal{S}$.


\begin{figure}[hbt]
\centering
\input{figure/tikz-palis-de-melo}
\caption{A plot of the zero set of the Palis-de Melo function, \cref{eqn-pdm}. The lines indicate the sets where the function is zero. The green line corresponds to $\inlinenorm{x}_2 = 1$; the black line corresponds to one branch of the zero set of the sinusoidal term (when $\inlinenorm{x}_2 > 1$); and the orange line corresponds to the another branch of the zero set of the sinusoidal term with a phase shift of $\pi$. The pluses and minuses indicate where $F$ is positive and negative, respectively. The two purple points correspond to $(1+\frac{1}{2\pi},0)$ and $(1+\frac{1}{\pi},0)$.} \label{figure-palis-de-melo-zero}
\end{figure}

\begin{figure}[hbt]
\centering
\input{figure/tikz-palis-de-melo-profile}
\caption{A profile plot of the Palis-de Melo function, \cref{eqn-pdm}, when $\cmp{x}{2} = 0$.} \label{figure-palis-de-melo-profile}
\end{figure}

\subsection{Spurious Solution for the Palis-de Melo Function} \label{subsection-pdm-spurious}

Now, suppose we apply gradient descent to any initialization with scalar step sizes satisfying \cref{property-spd,property-diverge,property-summable}, and that the iterates generated by gradient descent remain in $\mathcal{U}$. Then, the iterates are finite and \cref{result-zoutendjik-summable} implies that they must converge to a stationary point. Thus, we have a contradiction. To conclude, continuous gradient descent has a spurious solution for gradient descent with diminishing, summable step sizes. In other words, the properties of continuous gradient descent, \textit{regardless of our initialization}, do not all apply to gradient descent with diminishing, summable step sizes. 

While this proof is completely sufficient, we can provide some geometric insight into why we should expect this to hold. In particular, recall that we effectively need to spiral around the circle, $\mathcal{S}$, using a discrete method that only uses gradient information. As we get closer and closer to this circle, our gradient will be perpendicular to the circle and so, no matter our step size, we must deviate from the tracing of this circle.

==> section/global-convergence-sum.tex <==
In this section, we study the global convergence of gradient descent, \cref{eqn-recursion-iterate}, with diminishing step sizes with summability (\cref{property-spd,property-diverge,property-summable}), on a general class of nonconvex functions as defined by \cref{assumption-lower-bound,assumption-gradient}. As \cref{property-summable} implies \cref{property-diminishing}, \cref{result-zoutendjik} holds when we require the step sizes to satisfy \cref{property-spd,property-diverge,property-summable} in place of \cref{property-spd,property-diverge,property-diminishing}. However, owing to the greater stringency of \cref{property-summable}, we are able to strengthen the conclusions of \cref{result-zoutendjik}. In particular, we will prove that, when the iterates do not diverge, they \textit{converge} to a stationary point (see \cref{result-zoutendjik-summable}). Recall, when the iterates remain bounded in \cref{result-zoutendjik}, we do not conclude that the iterates must converge and we only show that the gradient function is arbitrarily close to zero infinitely often. 

To prove this strengthened result, we use an argument that is derived from common Borel-Cantelli arguments. Specifically, to establish that the gradient converges to zero, we study how frequently the gradient function jumps above an arbitrarily small value. We then count the number of times this can happen, and, using something akin to Markov's inequality, we prove that this count must be finite by using \cref{property-summable}. Similarly, to establish that the iterates will converge if they do not diverge, we study how frequently an iterate can remain within a bounded region of an arbitrary point in $\mathbb{R}^p$ and the next iterate can jump outside of this region. Again, using something akin to Markov's inequality, we prove that the number of times such a jump can happen is finite by using \cref{property-summable}. 

\subsection{Convergence of the Gradient}

One of the limitations of \cref{result-zoutendjik} is that it only states that the limit infimum of the gradient function goes to zero. By using \cref{property-summable} in place of \cref{property-diminishing}, we can show that the limit supremum agrees with the limit infimum, which we establish in the next result. 

\begin{theorem} \label{result-gradient-convergence}
Suppose $F:\mathbb{R}^p \to \mathbb{R}$ satisfies \cref{assumption-lower-bound,assumption-gradient}. Let $x_0 \in \mathbb{R}^p$ and let $\lbrace x_k : k \in \mathbb{N} \rbrace$ be generated by \cref{eqn-recursion-iterate} satisfying \cref{property-spd,property-diverge,property-summable}. Then, for all $ R \geq 0$,
\begin{equation}
\lim_{k \to \infty} \norm{ \dot F(x_k) }_2 \chi_k^0(R) = 0.
\end{equation}
Moreover, if $\sup_{k} \inlinenorm{ x_k}_2 < \infty$ then $\lim_{k \to \infty} \inlinenorm{ \dot F(x_k) }_2 = 0$.
\end{theorem}
\begin{proof}
By \cref{result-zoutendjik}, for every $R \geq 0$, $\liminf_{k} \inlinenorm{ \dot F(x_k) }_2 \chi_k^0(R) = 0$. For a contradiction, suppose $\exists \  \delta > 0$ such that $\limsup_{k} \inlinenorm{ \dot F(x_k) }_2 \chi_k^0(R) > \delta$. Then, for some $\gamma > 0$ sufficiently small, there exists a subsequence $\lbrace k_j : j \in \mathbb{N} \rbrace \subset \mathbb{N}$ such that $\inlinenorm{ \dot F(x_{k_j+1})}_2 \chi_{k_j+1}^0(R) \geq \delta + \gamma$ while $\inlinenorm{ \dot F(x_{k_j})}_2 \chi_{k_j}^0(R) \leq \delta$. Thus,
\begin{align*}
\delta + \gamma &\leq \norm{ \dot F(x_{k_j+1})}_2 \chi_{k_j+1}^0(R) \\
			   &\leq \norm{ \dot F(x_{k_j+1}) - \dot F(x_{k_j})}_2 \chi_{k_j+1}^0(R) + \norm{ \dot F(x_{k_j} }_2 \chi_{k_j+1}^0(R) \\
			   &\leq L(x_{k_j+1},x_{k_j}) \norm{ x_{k_j+1} - x_{k_j}}_2 \chi_{k_j + 1}^0(R) + \norm{ \dot F(x_{k_j})}_2 \chi_{k_j}^0(R) \\
			   &\leq L_R \norm{ M_{k_j} \dot F(x_{k_j})}_2 \chi_{k_j + 1}^0(R) + \delta \\
			   &\leq L_R \delta \lambda_{\max}(M_{k_j}) + \delta.
\end{align*}
Subtracting $\delta$ from both sides we have $\gamma < L_R \delta \lambda_{\max}(M_{k_j})$, from which it follows that $\gamma^q < L_R^q \delta^q \lambda_{\max}(M_{k_j})^q$, for $q\geq 0$. Summing over all $j$, $\sum_{j=1}^\infty \gamma^q < L_R^q \delta^q \sum_{j=1}^\infty \lambda_{\max}(M_{k_j})^q$. The sum on the left diverges while the sum on the right is finite by \cref{property-summable} for any appropriate choice of $q$, which leads to a contradiction. Hence, the limit supremum and the limit infimum must agree and the first conclusion of the statement follows.

% Subtracting $\delta$ from both sides, $\gamma < L_R \delta \lambda_{\max}(M_{k_j})$. Then, $\gamma^q < L_R^q \delta^q \lambda_{\max}(M_{k_j})^q$. By summing both sides over all $j$, $\sum_{j=1}^\infty \gamma^q < L_R^q \delta^q \sum_{j=1}^\infty \lambda_{\max}(M_{k_j})^q$. The sum on the left diverges whiles the sum on the right is finite by \cref{property-summable}, which is a contradiction. Hence, the limit supremum and the limit infimum must agree and the first conclusion of the statement follows.

Finally, when $\sup_{k} \inlinenorm{ x_k}_2 < \infty$, there exists an $R > 0$ such that $\chi_{k}^0(R) = 1$ for all $k+1 \in \mathbb{N}$, and thus the final conclusion of the statement follows.
\end{proof}


\subsection{Convergence of the Iterates}

Using a nearly identical argument as for the convergence of the gradient, we show that the iterates either converge to a point or they diverge. Again, \cref{property-summable} is essential to this conclusion.

\begin{theorem} \label{result-iterate-convergence}
Suppose $F:\mathbb{R}^p \to \mathbb{R}$ satisfies \cref{assumption-gradient}. Let $x_0 \in \mathbb{R}^p$ and let $\lbrace x_k : k \in \mathbb{N} \rbrace$ be generated by \cref{eqn-recursion-iterate} satisfying \cref{property-spd,property-summable}. Then, $\lbrace x_k : k+1 \in \mathbb{N} \rbrace$ converges to a fixed point or it diverges.
\end{theorem}
\begin{proof}
Let $z \in \mathbb{R}^p$. We study the sequence $\lbrace \inlinenorm{ x_k - z}_2 \rbrace$. Suppose for the purposes of a  contradiction that  $\exists \ R > 0$ such that $\liminf_k \inlinenorm{ x_k - z}_2 < R < \limsup_k \inlinenorm{ x_k - z}_2$. Then,  $\exists \ \gamma > 0$ and a subsequence $\lbrace k_j : j \in \mathbb{N} \rbrace$ such that $\inlinenorm{ x_{k_j} - z }_2 \leq R < R + \gamma \leq \inlinenorm{ x_{k_j + 1} - z }_2$. Notice,
\begin{align*}
R + \gamma 
&\leq \inlinenorm{ x_{k_j + 1} - z }_2 \\
&\leq \inlinenorm{ x_{k_j + 1 } - x_{k_j} }_2 + \inlinenorm{ x_{k_j} - z}_2 \\
&\leq \inlinenorm{ M_{k_j} \dot F(x_{k_j})}_2 + R \\
&\leq \lambda_{\max}(M_{k_j}) G_{R,z} + R,
\end{align*}
where $G_{R,z} = \max_{ x : \inlinenorm{x - z}_2 \leq R} \inlinenorm{ \dot F(x)}_2$, which is finite by continuity and compactness. Hence, $\gamma \leq \lambda_{\max}(M_{k_j}) G_{R,z}$. In particular, $\sum_{j=1}^\infty \gamma^q \leq G_{R,z}^q \sum_{j=1}^\infty \lambda_{\max}(M_{k_j})^q$, for $q\geq0$. The sum on the left hand side is infinite, while the sum on the right hand side is finite by \cref{property-summable} for any appropriate choice of $q$, which is a contradiction. Therefore, the limit supremum and limit infimum must agree.

This leaves two possibilities: $\lim_{k \to \infty} \inlinenorm{ x_k - z}_2$ is either infinite or finite. In the case that the limit is infinite, there is nothing more that we need to do as this implies that $\lbrace x_k \rbrace$ must diverge. In the case that the limit is finite, we can replace $z$ by any $p+1$ distinct points, $z_1,\ldots,z_{p+1} \in \mathbb{R}^p$, whose affine hull is $\mathbb{R}^p$. Then $\lim_{k \to \infty} \inlinenorm{x_k - z_j }_2 < \infty$ for $j=1,\ldots,p+1$. By triangulation, we conclude that $\lbrace x_k \rbrace$ must converge to a fixed point.
\end{proof}

Combining the conclusions of  \cref{result-zoutendjik,result-gradient-convergence,result-iterate-convergence}, we have the following summary.
\begin{corollary} \label{result-zoutendjik-summable}
Suppose $F:\mathbb{R}^p \to \mathbb{R}$ satisfies \cref{assumption-lower-bound,assumption-gradient}. Let $x_0 \in \mathbb{R}^p$ and let $\lbrace x_k : k \in \mathbb{N} \rbrace$ be generated by \cref{eqn-recursion-iterate} satisfying \cref{property-spd,property-diverge,property-summable}. Then, either $\lbrace x_k : k+1 \in \mathbb{N} \rbrace$ converges to a stationary point or diverges.
\end{corollary}
\begin{proof}
By \cref{result-iterate-convergence}, $\lbrace x_k \rbrace$ either converges to a point, $x^*$, or diverges. Moreover, if $\lbrace x_k \rbrace$ converges to $x^*$, then the iterates remain bounded.  By \cref{result-gradient-convergence} and \cref{assumption-gradient}, $\dot F(x_k) \to 0$ and $\dot F(x_k) \to \dot F(x^*)$, which implies $\dot F(x^*) = 0$. 
\end{proof}
